Bidirectional compression in heterogeneous settings for distributed or federated learning with partial participation: tight convergence guarantees

We introduce a framework - Artemis - to tackle the problem of learning in a distributed or federated setting with communication constraints and device partial participation. Several workers (randomly sampled) perform the optimization process using a central server to aggregate their computations. To alleviate the communication cost, Artemis allows to compress the information sent in both directions (from the workers to the server and conversely) combined with a memory mechanism. It improves on existing algorithms that only consider unidirectional compression (to the server), or use very strong assumptions on the compression operator, and often do not take into account devices partial participation. We provide fast rates of convergence (linear up to a threshold) under weak assumptions on the stochastic gradients (noise's variance bounded only at optimal point) in non-i.i.d. setting, highlight the impact of memory for unidirectional and bidirectional compression, analyze Polyak-Ruppert averaging. We use convergence in distribution to obtain a lower bound of the asymptotic variance that highlights practical limits of compression. We propose two approaches to tackle the challenging case of devices partial participation and provide experimental results to demonstrate the validity of our analysis.

==> boader-work.tex <==
\subsection{Broader Impact}
\label{sect:broadimpact}
\gs

\constantin{qu'est-ce qu'on fait de ce truc ?}

Our work is not directly targeted to any particular type of application. On the contrary, distributed learning is ubiquitous in the modern machine learning, and applications can range from NLP (training a test model on smartphones), to computer vision or medical applications.  Moreover, compression does not impact learning by itself or the nature of exchanged information; it only impacts \textit{the quality} and \textit{the weight} of the information exchanged: our goal is not to modify what is learned, but mostly to alleviate the learning process. As a consequence, the  impact of our work is inherently dependant on the applications for  which it will be used. Nevertheless, independently of the application, the algorithm has several impactful features.
\begin{enumerate}
    \item This work's first motivation is to reduce the communication cost.  Network usage has a huge environmental cost, requiring both a heavy and expensive infrastructure, and using an important amount of energy on a daily basis \citep{energy}. Moreover, it poses practical concerns for users in areas where bandwidth is limited. Overall \Artemis~alleviates the bandwidth requirement, thus lowering carbon  and environmental footprints, and improving accessibility.
    \item Moreover we tackle the non i.i.d.~setting which is a fundamental point to provide personalized models. This can substantially improve the adequacy of the model to the user. As mentioned before, the final impact of personalized models is also application-dependent: from medical applications to targeted ads on social media (for example, it could  even be used to manipulate voters to overbalance an election, see e.g.~\citep{bessi2016social}). 
    \item  More generally, this work is part of a common dynamic to improve  distributed algorithms. This  allows to generalize settings that keep the data on users' devices to preserve their privacy. Ultimately, the goal is to allow resources to be shared while preserving privacy.
\end{enumerate}

Overall, though the impact of such algorithms is expected to be positive, at least on energy/environmental concerns, cautiousness is still required, as a \textit{rebound} effect may be observed \citep{grubb1990communication}: having energetically cheaper and faster algorithms may result in an increase of such applications, annihilating the gain made by algorithmic progress.  

Inevitably, this requires to  carefully analyze the relevance of each situation in order to not systematize the  deployment of technological solutions when they are not required.
